AGS-GNN: Attribute-guided Sampling for Graph Neural Networks

We propose AGS-GNN, a novel attribute-guided sampling algorithm for Graph Neural Networks (GNNs) that exploits node features and connectivity structure of a graph while simultaneously adapting for both homophily and heterophily in graphs. (In homophilic graphs vertices of the same class are more likely to be connected, and vertices of different classes tend to be linked in heterophilic graphs.) While GNNs have been successfully applied to homophilic graphs, their application to heterophilic graphs remains challenging. The best-performing GNNs for heterophilic graphs do not fit the sampling paradigm, suffer high computational costs, and are not inductive. We employ samplers based on feature-similarity and feature-diversity to select subsets of neighbors for a node, and adaptively capture information from homophilic and heterophilic neighborhoods using dual channels. Currently, AGS-GNN is the only algorithm that we know of that explicitly controls homophily in the sampled subgraph through similar and diverse neighborhood samples. For diverse neighborhood sampling, we employ submodularity, which was not used in this context prior to our work. The sampling distribution is pre-computed and highly parallel, achieving the desired scalability. Using an extensive dataset consisting of 35 small ($\le$ 100K nodes) and large (>100K nodes) homophilic and heterophilic graphs, we demonstrate the superiority of AGS-GNN compare to the current approaches in the literature. AGS-GNN achieves comparable test accuracy to the best-performing heterophilic GNNs, even outperforming methods using the entire graph for node classification. AGS-GNN also converges faster compared to methods that sample neighborhoods randomly, and can be incorporated into existing GNN models that employ node or graph sampling.

==> 1Abstract-saved.tex <==
\begin{abstract}
%\Sid{ICML'24 (8-page main text, bibliography, and appendix unlimited after main text). The abstract must be limited to one paragraph.}

In homophilic graphs, vertices of the same class are more likely to be connected, and vertices of different classes tend to be linked in heterophilic graphs. While Graph Neural Networks (GNN) have been successfully applied to homophilic graphs, their application to heterophilic graphs remains challenging. Best-performing GNNs for heterophilic graphs do not support mini-batching, suffer high computational costs, and are not inductive.
We propose \ags{}, a novel attribute-guided sampling algorithm for GNNs that exploits node features and connectivity structure of a graph while simultaneously adapting for both homophily and heterophily in graphs. 
We employ feature-similarity and feature-diversity samplers to select a subset of neighbors for a node and adaptively capture information from homophilic and heterophilic neighborhoods using dual channels.
\ags{} works on the assumption that similarity in features and labels is positively correlated, and in the absence of an appropriate feature similarity metric, we employ a learning-based approach. Currently, \ags{} is the only algorithm that explicitly manipulates homophily in the sampled subgraph through similar and diverse neighborhood samples. We use similarity and marginal gains (from submodular function) based ranking of neighbors of a node and an appropriate probability density function to select similar and diverse samples. Our pre-computation step to estimate sampling probabilities is parallel and can be scaled to large graphs. 
Using an extensive dataset consisting of 35 small (less than 100K nodes) and large (>100K nodes) homophilic and heterophilic graphs, we demonstrate the superiority of \ags{}  relative to current approaches in the literature. \ags{} achieves comparable test accuracy to the best-performing heterophilic GNNs in the literature, even outperforming methods that use an entire graph at once for node classification. \ags{} also achieves faster convergence compared to GraphSAGE, which samples neighborhoods randomly. Additionally, \ags{} can be easily incorporated into existing GNN models using node or graph sampling. 
We therefore believe that \ags{} will significantly advance the application of GNNs for both heterophilic and homophilic graphs.
\end{abstract}


\begin{comment}
Graph Neural Network (GNN) has been successfully applied
to graphs under homophily and heterophily; however, training a large-scale GNN remains challenging for graphs with heterophily, and only a few exist in the literature. Some of the best-performing GNNs for heterophilic graphs do not support mini-batching, suffer a high computational cost, and are transductive.
In this paper, we propose \ags{}, a novel attribute-guided sampling algorithm for GNNs that exploits the feature and structure of the graph and is suitable for graphs under homophily and heterophily. \ags{} uses ego-neighborhood feature similarity and diversity-based sampler to select a subset of neighbors and adaptively captures information from homophilic and heterophilic neighborhoods using dual channels. \ags{} works on the assumption that similarity in features and labels is positively correlated, and in the absence of an appropriate feature similarity metric, we can learn one. \ags{} is the only algorithm that explicitly manipulates homophily in the sampled subgraph through similar and diverse ego-neighborhood samples. Our method uses similarity and marginal gains (from submodular function) based ranking of neighbors of a vertex and appropriate probability density function for selecting similar and diverse samples.
\ags{} comes with a pre-computation step of estimating the sampling probability of the edges that is scalable and can be computed in parallel for large graphs.
\ags{} offers node sampling and graph sampling techniques to incorporate with existing GNNs easily.
We experimented with $35$ benchmark datasets consisting of both small (vertices less than $100K$) and large (vertices more than $100K$) homophilic and heterophilic graphs, and found \ags{} to be among the top performing in all of these. 
\ags{} achieves comparable test accuracy to the best-performing heterophilic GNNs in the literature and even outperforms methods that use an entire graph at once. \ags{} also has faster convergence compared to GraphSAGE, which samples neighborhoods randomly.
\end{comment}


==> 2Introduction.tex <==
\section{Introduction}

The Graph Neural Network (GNN) works under the homophily assumption, which assumes most of the neighboring vertices of a vertex are similar. However, in practice~\citep{zheng2022graph}, we see graphs with different ranges of homophily scores~\citep{platonov2022characterizing}. 
When dealing with graphs with a low homophily score, termed heterophilic (definition \S\ref{subsec:homophiliydefinition}), GNNs often fail due to noisy or improper neighborhood aggregation \citep{luan2022revisiting}. 
The authors in~\citep{lim2021large, zhu2020beyond,  liu2021non,luan2020complete, chien2020adaptive} verify that even a simple Multi-Layer Perceptron (MLP) based model (e.g., LINKX) could outperform GNNs for mini-batch training on broad classes of heterophilic graphs. %This is because heterophilic graphs require exploring more relationships between ego-neighbor node features.

Currently, heterophilic GNNs~\citep{zheng2022graph,luan2022revisiting, zhu2020beyond,  liu2021non,luan2020complete, chien2020adaptive, zhu2021graph, yan2022two,li2022finding,xu2023node} are getting attraction as they appear in practice. However, most are generally trained on relatively small graphs, limiting their ability to model large-scale data and explore more complicated heterophilic patterns. The primary bottleneck of these heterophilic methods is their inability to perform mini-batch or subgraph sampling settings, thus not scaling well for arbitrarily large graphs and not being inductive. 
LINKX~\citep{lim2021large} is one of the notable scalable GNNs for heterophilic graphs in the literature; however, this method is transductive, and the MLP dimension depends on the number of nodes, which does not scale to massive graphs. 
%sid: moved this to related work
%Comparable to the LINKX, another recent scalable GNN, LD2~\citep{liao2023ld}, uses the pre-computation step to transform the adjacency matrix and input feature matrix into embeddings, then apply feature transformation in a mini-batch fashion on the embeddings. 


Recent works from~\citep{platonov2023critical, ma2021homophily} investigate some current benchmark heterophilic graphs and propose some new datasets where they have shown existing homophilic GNNs (with some customization) can perform as well as specialized GNNs designed for heterophily graphs. 
Thus, one possible solution to tackle scalability in certain heterophilic graphs is to apply mainstream sampling strategies of homophilic GNNs. 
However, current scalable homophilic GNNs~\citep{hamilton2017inductive, zeng2019graphsaint,chen2018stochastic,chen2018fastgcn,huang2018adaptive,chiang2019cluster}
%most sampling strategies or sparsification methods~\citep{srinivasa2020fast}
do not consider the underlying homophily of the graph. 
%Instead, the goal of these sampling strategies mainly focuses on taking unbiased random samples of the original graph. 
These homophilic GNNs undermine the connections and relationships of heterophilic nodes, mainly when similar and dissimilar neighbors contribute differently to learning the ego-node representations.
Another limitation of these sampling or sparsification techniques is that they only focus on the graph's structure, leaving out the feature information (node/edge features) for the downstream GNN models. %For high-quality samples, it is necessary to consider the graph's attributes and structure. Based on the assumption that the nodes with {\em similar features} tend to have a {\em similar label} (\S\ref{subsec:featurevslabel}), we propose an Attribute-Guided Sampling (AGS) framework for homophilic and heterophilic graphs. We find that taking biased samples (based on features and graph topology together) of the graph can learn a better representation of the graph for downstream tasks, improve the overall computation time of the training and inference process, achieve faster convergence, become more robust to noise, and increase the accuracy of predictions.
% We also show that with appropriate samplers, we can handle some heterophilic graphs using homophilic GNNs to some extent.
In this paper, we propose feature similarity and feature diversity-based samplers and show that changing the homophily of the sampled subgraphs through the feature-based sampling process can be more beneficial than random selection (\S\ref{subsec:prelimhomophily}). 
The similar neighborhood subgraphs are more robust to noise during training, and diverse neighborhoods help map heterophilic nodes of the same label to the same vector space. 
We adopted AGS into node and graph sampling paradigms and used existing GNNs. We use two channels with subgraphs of similar and diverse neighborhood samples and use MLPs to learn from which neighbors it should take the information. 

%We sample $k$ hop neighborhood in node sampling based on pre-computed weighted graphs. In addition to the weighted random walk-based subgraph selection for graph sampling, we compute disjoint sparse subgraphs (\S\ref{subsec:graph_sampling}). Here, we split the pre-computed weighted graph into a collection of the edge-disjoint subgraph of different properties (e.g., connectivity, regularity). We sample from these subgraphs and combine them to get a sparse graph for an epoch.

\textbf{Contributions:} The key contribution and findings of this work are summarized as follows:

\begin{enumerate}    
    \item We propose a novel scalalbe unsupervised and supervised feature-guided sampling framework that learns improved representation across homophilic and heterophilic graphs.
    Our proposed \ags{} is a scalable method for heterophilic graphs working under inductive settings.

    \item \ags{} %is the first work that uses submodular optimization for heterophilic graphs in the context of node neighborhood diversity. 
    incorporates sampling based on similarity and diversity, which is modeled by submodular function. To  the best of our knowledge, this is the first work that uses submodularity in the context of sampling.
    
    %All our pre-computation steps are local, performed to individual vertices, can be computed in parallel, and scale well for massive graphs. %Our novel edge-disjoint subgraph computations and the graph sampling techniques are adaptable to various customizations, catering to different problem requirements.

    \item For a node, \ags{} employs dual channels with MLPs to acquire knowledge from its feature-based similar and diverse neighborhood.

    \item We conducted a thorugh experiment with $35$ benchmark datasets for node classification and compared them against arrays of standard heterophilic and homophilic GNNs.
    For both heterophilic and homophilic graphs, \ags{} achieved improved performance than the competing methods (Fig.~\ref{fig:perfplot}). 
    In some datasets, sampled subgraphs of \ags{} even perform better than using the entire graphs (\S\ref{subsec:ablation_study}). \ags{} also requires fewer iterations (up to $50\%$ less) (\S\ref{subsec:runtimeandconvergence}) to converge than traditional methods while achieving improved or comparable results.
\end{enumerate}

% Section~\ref{sec:prelim} provides preliminaries on homophily and heterophily. Section~\ref{sec:method} comprehensively explains our proposed \ags{} framework. Section~\ref{sec:experiments} covers the experimental settings, results, and ablation study. Section~\ref{subsec:related_works} covers related works in the literature. Finally, Section~\ref{sec:conclusion} addresses the limitations of our approach, and explores future possibilities. Additional results and analysis have been relocated to the Appendix for conciseness.


\begin{comment}
\begin{enumerate}
\item \textbf{Pre-computation:} If we have the domain knowledge, we can use the appropriate similarity measure to rank neighbors of each vertex based on the associated node features using Nearest Neighbor, and Submodular functions (\S\ref{subsubsec:precompnodesample}). %(\S\ref{alg:nnweights}\S\ref{alg:subweights}). 
    In absence of domain knowledge, we use a learnable edge weight prediction (Alg.~\ref{alg:learnweights}) on the training subgraph to rank the neighborhood of a vertex.
    
    
    \item \textbf{Node Sampling:} Aggregation of attribute-guided samples of the neighborhood of vertices are of better quality (evaluated in terms of F1-Score) than random selection of neighbors (Table~\ref{tab:hetero_sub_vs_nn_rand}). With biased sampling, the GNN requires fewer iterations than the use of random sampling (Table ~\ref{tab:node_sampling_results}, ~\ref{tab:homophilic_graph}).

    \item \textbf{Graph Sampling:} From the pre-computed ranked graph, we can use weighted random walk to sample subgraphs for training. However, we can split graphs into disjoint subgraphs based on heuristic or learned weights to ensure connectivity and other properties in the sparse graph. Sample a few of these subgraphs, and combine them along with weighted random walks samples to get a sparse representation of the graph. We have found better performance (Algorithm~\ref{alg:disjointgraph}, Table~\ref{table:disjointgraph})

    \item For graphs with high homophily, random selection or Nearest Neighbor gives similar performance. However, for dense graphs with high homophily, maintaining diversity using sub-modular makes the sparse selection robust and achieves good performance with fewer iterations (Table~\ref{} \textbf{pending}).

    \item \textbf{\ags{}:} The heterophily of nodes can be useful sometimes for classification. Multiple vertices can be similar because of their same dissimilar neighborhood. The submodular samples of a vertex encourage diversity among neighboring features thus encouraging heterophily. Therefore, for a particular node, the combination of two types of samples (Nearest Neighbor samples), (Submodular Samples) can be useful for heterophilic graphs where we don't know which to consider. Additionally,  in certain scenarios, a decision without considering the neighborhood is also useful. Recent works~\cite {} also show that the Low pass filter representation of the graph (Laplacian, Chebyshev) is useful for the heterophilic graph. 

    In the second part of \ags{} framework, we design a GNN that contains two channels~\footnote{We can have multiple channels and their corresponding message passing networks}, where one takes homophilic and the other takes heterophilic samples from seed nodes and use the corresponding GNN to get the representations. Finally, another MLP on top of it acts as a decision layer to decide which representation to consider.  \ags{} demonstrates improved performance in heterophilic datasets (\S\ref{sec:AGSGNN}).
\end{enumerate}
\end{comment}

==> 7.1submodularity.tex <==
\subsection{Submodular Selection and Diversity}
\label{subsec:submodular_diversity}

%AP: do we really need this subsection? This material reads like a tutorial, not a paper.

%sid: removed from the appendix


A submodular function is a set valued function that assigns a value to every subset of a ground set that satisfies the diminishing returns property, i.e., for two subsets $S$, $T$ with $S\subseteq T$ of a ground set $A$, and any  element $e \in A\setminus T$, 
$$f(S\cup{e}) - f(S) \geq f(T\cup{e}) - f(T).$$
 An example of a submodular function is  the facility location function
\begin{equation}
    f(S, A) = \sum\limits_{y\in A} \max_{x\in S} \phi(x, y), 
    \label{eq:facility_location_function}
\end{equation}
where $S$ and $A$ are as above  and $\phi$ is a  similarity measure on the elements of $A$. The quantity on either side of the inequality is the \emph{marginal gain}. 
The facility location function can be maximized by %we find a subset of elements that maximizes the function value and can b
a Greedy algorithm, which starts with the empty subset and iteratively adds an element that gives the largest marginal gain to the function value until a cardinality  (or other) constraint on $S$ is reached. 
%The process is similar to $k$-medoid clustering; after the first few examples are selected, the subsequent ones are at the center of clusters.

To illustrate, let us have seven points with two-dimensional features to demonstrate the selection strategy. Here, we added $0$ to the $y$-axis to show that all points fall in a line in the $x$-axis and become more accessible to visualize (Fig.~\ref{fig:submodular_line}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!htbp]
 \centering
 \includegraphics[width=1.0\linewidth, angle = 0 ]{Figures/Prelimilaries/line_feature.pdf}
 \caption{Features of the data points.}
 \label{fig:submodular_line}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\[ \mX =
\begin{bmatrix}
0 & 0\\
1 & 0\\
2 & 0\\
5 & 0\\
7 & 0\\
8 & 0\\
9 & 0
\end{bmatrix}
\]

We compute $distance^2.max()-distance^2$ to convert the Euclidean distance to similarity. Squared Euclidean distance is used in practice since it is faster, and the relative order of selection does not change. Then we get the following similarity measures between these points, 

\[ \phi =
\begin{bmatrix}
81 & 80 & 77 & 56 & 32 & 17 & 0\\
80 & 81 & 80 & 65 & 45 & 32 & 17\\
77 & 80 & 81 & 72 & 56 & 45 & 32\\
56 & 65 & 72 & 81 & 77 & 72 & 65\\
32 & 45 & 56 & 77 & 81 & 80 & 77\\
17 & 32 & 45 & 72 & 80 & 81 & 80\\
0 & 17 & 32 & 65 & 77 & 80 & 81\\
\end{bmatrix}
\]

\begin{enumerate}

\item The ground set is $A=\{1,2,3,4,5,6,7\}$ is same in all steps.  The subset is $S=\{\}$ in the first step.
From the eq.~\ref{eq:facility_location_function} we can see for the first element, $S=\{i\}$, the equation reduces to,
\begin{equation*}
f(\{i\}, A) - f(\{\},A) = \sum\limits_{y\in A} \phi(x_i, x_y) - 0    
\end{equation*}

This is the summation of rows for the marginal gain, meaning the point that stays far from all points will have maximum marginal gain. In this case, that is the $4$th data point with marginal gain $488$ (summation of $4$th row from $\phi$). The $4$th point with the feature $[5, 0]$ resides close to the middle of the line.

\item In the second step, we have $S=\{4\}$ and $A=\{1,2,3,4,5,6,7\}$. 
The marginal gain is, 
\begin{align*}
f(\{4\}\cup \{i\}, A) - f(\{4\},A) = \\\sum\limits_{y\in A} \max(\phi(x_4, x_y),\phi(x_i, x_y)) - 488    
\end{align*}

For an element $i$, this computes the column-wise maximum between its row and row of the $4$th element and subtracts the gain with the selected element. This computation tries to find a point farther from element $4$ and maximizes respect to others. We get the $2$nd element with a marginal gain of $48$. This is because feature $[1,0]$ can be considered a cluster centroid farther from $[5,0]$.

\item In the third step, we will select $6$th element, and then at later steps, we will select element  $1, 3, 5, 7$ in order. 
Therefore, the final order of elements by marginal gains becomes $[4, 2, 6, 1, 3, 5, 7]$, representing their diversity contribution in order.

\end{enumerate}

Intuitively, the function tends to select points far from each other since this increases the similarity between each point and its nearest chosen point. For example, suppose the function has already chosen a point that is very similar to many other points. In that case, adding another point that is also very similar to those points will not increase the function value much since the similarity between those points and their nearest chosen point will remain the same. However, adding a point very different from the already chosen points will increase the function value more since the similarity between that point and its nearest chosen point will be higher than the similarity between that point and any other chosen point.

It means that the successively chosen examples are representative of underrepresented examples. The function tries to find a subset of points that covers the diversity of the whole set of points. For example, suppose the points contain points from different categories, such as animals, plants, and minerals. In that case, the function will try to choose points belonging to different categories, representing each category at least one point in the subset. This way, the function captures the essence of the whole set of points with a smaller subset of points.

In our context, $S$ is the current set of selected nodes initialized with ego node $t$, and ground set $A = \gN(t)\cup \{t\}$. 
Marginal gains for neighbors are $f_i = f(S\cup \{i\},A)-f(S,A)$ for each neighbor $i\in \gN(t)\setminus S$.  The neighbors are incrementally added based on marginal gain. 
Since we assume features and labels are positively correlated, we can expect the diverse neighbors in terms of features will result in a diverse neighborhood in terms of labels. 


\textbf{Observation:} \textit{Starting with initial set $S=\{t\}$, selecting subset of neighbors, $\gN(t)$, of an ego node $t$ based on marginal gains of submodular function, $f(S, A) = \sum_{y\in A} \max_{x\in S} \phi(x, y)$ results a diverse neighborhood. }   


    

% Intuitively, the function $f(S,A)$ encourages selecting neighbors that are far from each other, since this increases the similarity between selected nodes and its nearest chosen neighbor. For example, When $S$ is an ego node only, then $f(S,A)$ is the maximum similarity between all neighbor points in $A$ and the ego node $S$. If S contains two points that are far apart, then f(S,A) is the sum of the maximum similarities between each point in A and its closest point in S. This is likely to be larger than the previous case, since each point in A has a higher chance of being close to one of the points in S.

==> Experiments/Ablation.tex <==
%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htbp]
\centering
\resizebox{0.7\linewidth}{!}{
\def\arraystretch{1.2}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Degree} & \textbf{N} & \textbf{E} & \textbf{Rand-it} & \textbf{Rand-acc} & \textbf{NN-it} & \textbf{NN-acc} & \textbf{Sub-it} & \textbf{Sub-acc} \\ \hline
10  & 2708 & 27079  & 99  & 0.8802 & 59  & 0.8934 & 64 & 0.8745 \\ \hline
20  & 2708 & 40619  & 98  & 0.8811 & 65  & 0.9016 & 72 & 0.8852 \\ \hline
30  & 2708 & 54159  & 93  & 0.8824 & 71  & 0.9119 & 78 & 0.8917 \\ \hline
40  & 2708 & 67699  & 103 & 0.8878 & 76  & 0.9169 & 76 & 0.8932 \\ \hline
50  & 2708 & 81239  & 102 & 0.8876 & 84  & 0.9201 & 81 & 0.8966 \\ \hline
60  & 2708 & 94779  & 100 & 0.8875 & 83  & 0.9230 & 88 & 0.8995 \\ \hline
70  & 2708 & 108319 & 103 & 0.8876 & 92  & 0.9257 & 95 & 0.901  \\ \hline
80  & 2708 & 121859 & 102 & 0.8869 & 93  & 0.9269 & 94 & 0.9018 \\ \hline
90  & 2708 & 135399 & 105 & 0.8892 & 96  & 0.9280 & 98 & 0.9037 \\ \hline
100 & 2708 & 148939 & 107 & 0.89   & 100 & 0.9295 & 99 & 0.905  \\ \hline
\end{tabular}
}
\caption{Node sampling performance on Synthetic Cora dataset with homophily score of 0.8 and varying degree.}
\end{table}
%%%%%%%%%%%%%%%%%%%


\begin{table}[htbp]
\centering
\resizebox{1.0\linewidth}{!}{
\def\arraystretch{1.5}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{ACMGCNP-   Struc} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} &
  \textbf{} \\ \hline
\textbf{Dataset} &
  \textbf{Nh} &
  \textbf{Eh} &
  \textbf{EiH} &
  \textbf{Degree} &
  \textbf{N} &
  \textbf{E} &
  \textbf{Original} &
  \textbf{Rand Nh} &
  \textbf{Rand Acc} &
  \textbf{NN Nh} &
  \textbf{NN Acc} &
  \textbf{Sub Nh} &
  \textbf{Sub Acc} &
  \textbf{Link NN Nh} &
  \textbf{Link NN Acc} &
  \textbf{Link Sub Nh} &
  \textbf{Link Sub Acc} \\ \hline
cornell &
  0.21 &
  0.31 &
  0.06 &
  1.63 &
  183 &
  298 &
  0.8162 &
  0.29 &
  0.8757 &
  0.34 &
  0.8216 &
  0.24 &
  0.8162 &
  0.32 &
  0.8378 &
  0.27 &
  0.773 \\ \hline
texas &
  0.07 &
  0.11 &
  0.00 &
  1.78 &
  183 &
  325 &
  0.8595 &
  0.10 &
  0.8919 &
  0.13 &
  0.8757 &
  0.09 &
  \textbf{0.9243} &
  0.13 &
  0.8378 &
  0.09 &
  0.8757 \\ \hline
wisconsin &
  0.17 &
  0.20 &
  0.08 &
  2.05 &
  251 &
  515 &
  0.8941 &
  0.15 &
  0.8784 &
  0.19 &
  0.8902 &
  0.12 &
  \textbf{0.8941} &
  0.15 &
  0.8824 &
  0.16 &
  0.8863 \\ \hline
squirrel &
  0.09 &
  0.22 &
  0.04 &
  41.74 &
  5201 &
  217073 &
  0.7635 &
  0.22 &
  0.4722 &
  0.25 &
  0.5091 &
  0.21 &
  \textbf{0.5695} &
  0.25 &
  0.557 &
  0.20 &
  0.5091 \\ \hline
chameleon &
  0.10 &
  0.24 &
  0.06 &
  15.85 &
  2277 &
  36101 &
  0.7715 &
  0.25 &
  0.6289 &
  0.28 &
  0.6289 &
  0.25 &
  \textbf{0.643} &
  0.41 &
  0.6294 &
  0.13 &
  0.5939 \\ \hline
\textbf{ACMGCN} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \hline
\textbf{Dataset} &
  \textbf{Nh} &
  \textbf{Eh} &
  \textbf{EiH} &
  \textbf{Degree} &
  \textbf{N} &
  \textbf{E} &
  \textbf{Original} &
  \textbf{Rand Nh} &
  \textbf{Rand Acc} &
  \textbf{NN Nh} &
  \textbf{NN Acc} &
  \textbf{Sub Nh} &
  \textbf{Sub Acc} &
  \textbf{Link NN Nh} &
  \textbf{Link NN Acc} &
  \textbf{Link Sub Nh} &
  \textbf{Link Sub Acc} \\ \hline
cornell &
  0.21 &
  0.31 &
  0.31 &
  1.63 &
  183 &
  298 &
  0.7459 &
  0.31 &
  0.6378 &
  0.34 &
  0.7081 &
  0.24 &
  \textbf{0.6703} &
  0.38 &
  0.7297 &
  0.21 &
  0.7027 \\ \hline
texas &
  0.07 &
  0.11 &
  0.11 &
  1.78 &
  183 &
  325 &
  0.8432 &
  0.11 &
  0.8108 &
  0.13 &
  0.7405 &
  0.09 &
  \textbf{0.8541} &
  0.14 &
  0.8108 &
  0.08 &
  0.7946 \\ \hline
wisconsin &
  0.17 &
  0.20 &
  0.20 &
  2.05 &
  251 &
  515 &
  0.8627 &
  0.15 &
  0.7961 &
  0.19 &
  0.7804 &
  0.12 &
  \textbf{0.851} &
  0.18 &
  0.8275 &
  0.13 &
  0.8039 \\ \hline
squirrel &
  0.09 &
  0.22 &
  0.22 &
  41.74 &
  5201 &
  217073 &
  0.5066 &
  0.22 &
  0.4359 &
  0.25 &
  0.4434 &
  0.21 &
  \textbf{0.4795} &
  0.28 &
  0.4857 &
  0.17 &
  0.474 \\ \hline
chameleon &
  0.10 &
  0.24 &
  0.24 &
  15.85 &
  2277 &
  36101 &
  0.6579 &
  0.25 &
  0.5969 &
  0.28 &
  0.6123 &
  0.25 &
  \textbf{0.6079} &
  0.44 &
  0.5912 &
  0.11 &
  0.5917 \\ \hline
\end{tabular}

}

\caption{Performance comparison of single instance of sparse graph in graph with heterophily}
\label{tab:hetero_sub_vs_nn_rand}
\end{table}

==> Experiments/AblationResults.tex <==
% %with +/
% \begin{table}[!htbp]
% \centering
% \resizebox{1.0\linewidth}{!}
% {
% \def\arraystretch{1.2}
% \begin{tabular}{l|c|c|c|c|c|c}
% \toprule
% Dataset             & \multicolumn{2}{c|}{CoraSyn0.05}   & \multicolumn{2}{c|}{CoraSyn0.25}   & \multicolumn{2}{c}{CoraSyn0.50}                  \\\midrule
% GNN & GSAGE & ChebNet & GSAGE & ChebNet & GSAGE &ChebNet \\\midrule
% Random & 57.08 $\pm$ 0.46 & 56.44 $\pm$ 0.14 & 61.85 $\pm$ 0.94 & 62.14 $\pm$ 1.29 & 92.09 $\pm$ 0.79 & 92.48 $\pm$ 0.72 \\
% NN & 48.50 $\pm$ 0.29 & 50.91 $\pm$ 0.22 & \textbf{71.66} $\pm$ 0.42 & \textbf{71.02} $\pm$ 0.17 & 92.48 $\pm$ 0.51 & 91.71 $\pm$ 0.25 \\
% Sub & 61.79 $\pm$ 0.17 & \textbf{64.67} $\pm$ 0.22 & 53.91 $\pm$ 0.22 & 57.03 $\pm$ 0.30 & 79.48 $\pm$ 0.36 & 76.07 $\pm$ 0.36 \\
% Whole & \textbf{63.67} $\pm$ 0.43 & 62.79 $\pm$ 0.25 & 69.49 $\pm$ 0.38 & 67.61 $\pm$ 0.22 & \textbf{96.94} $\pm$ 0.08 & \textbf{96.47} $\pm$ 0.14\\\bottomrule
% \end{tabular}
% }
% \caption{$F_1$ score of a single sparse subgraph keeping $25\%$ of the original neighborhood from the original graph. Here, three synthetic versions of Cora are produced with degree $d = 200$ and node homophily $0.05, 0.25$, and $0.50$, respectively. We compare Nearest Neighbor and Submodular sparsification against random and whole graphs with underlying GSAGE and ChebNet.}
% \label{tab:corasynsparse}
% \end{table}
% %%%%%%%%%%%%%
% \begin{table}[!htbp]
% \centering
% \resizebox{1\linewidth}{!}
% {
% \def\arraystretch{1.2}
% \begin{tabular}{l|c|c|c|c|c|c}
% \toprule
% Dataset & \multicolumn{2}{c|}{CoraSyn0.05} & \multicolumn{2}{c|}{CoraSyn0.25} & \multicolumn{2}{c}{CoraSyn0.50} \\\midrule
% GNN & GSAGE & 
% ChebNet & GSAGE & ChebNet & GSAGE & ChebNet \\\midrule
% Random & 59.20 $\pm$ 0.22 & 57.50 $\pm$ 0.80 & 62.85 $\pm$ 0.55 & 61.67 $\pm$ 0.46 & 91.06 $\pm$ 0.36 & 88.89 $\pm$ 1.32 \\
% NN & 54.44 $\pm$ 0.68 & 54.03 $\pm$ 0.51 & \textbf{69.19} $\pm$ 0.08 & \textbf{67.43} $\pm$ 0.30 & \textbf{92.00} $\pm$ 0.08 & \textbf{91.71} $\pm$ 0.29 \\
% Sub & \textbf{60.96} $\pm$ 0.55 & \textbf{61.73} $\pm$ 0.43 & 56.67 $\pm$ 0.46 & 58.38 $\pm$ 0.25 & 86.65 $\pm$ 0.44 & 83.54 $\pm$ 0.79
% \\\bottomrule
% \end{tabular}
% }
% \caption{$F_1$ score with a differently weighted sampler that generates sparse subgraphs. Here are three synthetic versions of Cora with degree $d = 200$ and node homophily $0.05$, $0.25$, and $0.50$. Underlying GNNs are GSAGE and ChebNet.}
% \label{tab:corasynsampler}
% \end{table}
% %%%%%%%%%%%%%




% \begin{table}[htbp]
% \centering
% \resizebox{0.5\linewidth}{!}
% {
% \def\arraystretch{1.0}
% \begin{tabular}{l|cc}
% \toprule
% GNNs     & \multicolumn{2}{c}{CoraSyn} \\
% %GNNs & \multicolumn{2}{c}{GSAGE+ChebNet}          \\\midrule
% \textbf{}   & $\mu$                & $\sigma$            \\\midrule
% ACM-GCN         & 35.34          & 0.69          \\
% LINKX       & 34.21          & 0.79          \\
% Whole graph & 60.50          & 1.14          \\
% % Rand+Random & 60.41          & 0.77          \\
% AGS (NN + NN)     & 60.81          & 0.78          \\
% AGS (Sub + Sub)   & 62.84          & 0.85          \\
% AGS (NN + Sub)    & \textbf{63.03} & \textbf{0.51}\\\bottomrule
% \end{tabular}
% }
% \caption{$F_1$ Score of two-channel GNNs with a differently weighted sampler in synthetic Cora graph with locally heterophilic and homophilic nodes mixed ($h_n(u) =[0.05,0.50])$.}
% \label{tab:coratwochannel}
% \end{table}

==> Experiments/Alldataset.tex <==

\begin{table*}[htbp]
\centering
\resizebox{1.0\linewidth}{!}{
\def\arraystretch{1.2}
\begin{tabular}{l|cccccccccccccccc|c}
\hline
\textbf{Dataset} &
  \textbf{N} &
  \textbf{E} &
  \textbf{d} &
  \textbf{Nh} &
  \textbf{Eh} &
  \textbf{Ch} &
  \textbf{A} &
  \textbf{Set} &
  \textbf{Iteration} &
  \textbf{GSAGE} &
  \textbf{Set} &
  \textbf{Interation} &
  \textbf{Cheb} &
  \textbf{Set} &
  \textbf{Iteration} &
  \textbf{AGS-GNN} &
  \textbf{Comment} \\\hline
Actor &
  7600 &
  30019 &
  3.95 &
  0.1586 &
  0.2188 &
  0.0061 &
  -0.1111 &
  8,4 &
  150 &
  0.3458 &
  8,4 &
  150 &
  0.35934 &
  4,4 &
  150 &
  \textbf{0.3678} &
   \\
Cornell &
  183 &
  298 &
  1.63 &
  0.1057 &
  0.1309 &
  0.1504 &
  -0.3836 &
  8,4 &
  57 &
  0.6486 &
  8,4 &
  101 &
  0.71351 &
  4,4 &
  77 &
  \textbf{0.7297} &
   \\
Texas &
  183 &
  325 &
  1.78 &
  0.0654 &
  0.1077 &
  0.0000 &
  -0.3463 &
  8,4 &
  54 &
  0.7838 &
  8,4 &
  92 &
  0.8 &
  4,4 &
  66 &
  \textbf{0.8919} &
   \\
Wisconsin &
  251 &
  515 &
  2.05 &
  0.1719 &
  0.1961 &
  0.0839 &
  -0.2723 &
  8,4 &
  56 &
  0.7451 &
  8,4 &
  107 &
  0.77255 &
  4,4 &
  76 &
  \textbf{0.8824} &
   \\
Chameleon &
  2277 &
  36101 &
  15.85 &
  0.1039 &
  0.2350 &
  0.0586 &
  -0.1128 &
  8,4 &
  141 &
  0.5219 &
  8,4 &
  150 &
  0.50965 &
  4,4 &
  150 &
  \textbf{0.6579} &
   \\
Squirrel &
  5201 &
  217073 &
  41.74 &
  0.0889 &
  0.2239 &
  0.0430 &
  0.3738 &
  8,4 &
  128 &
  0.3833 &
  8,4 &
  144 &
  0.37157 &
  4,4 &
  116 &
  \textbf{0.4476} &
   \\
Crocodile &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  Regression \\
penn94 &
  41554 &
  2724458 &
  65.56 &
  0.4828 &
  0.4704 &
  -1.0000 &
  -0.0013 &
  8,4 &
  30 &
  0.7606 &
  8,4 &
  116 &
  \textbf{0.76569} &
  4,4 &
  66 &
  0.7598 &
   \\
reed98 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  error \\
amherst41 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  error \\
cornell5 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  error \\
johnshopkins55 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  error \\
genius &
  4E+05 &
  984979 &
  2.33 &
  0.4774 &
  0.6176 &
  0.2170 &
  -0.1065 &
  8,4 &
  150 &
  0.8295 &
  8,4 &
  150 &
  0.82629 &
  4,4 &
  33 &
  0.8289 &
   \\
Roman-empire &
  22662 &
  65854 &
  2.91 &
  0.046 &
  0.0469 &
  0.0208 &
  -0.0282 &
  8,4 &
  150 &
  0.7643 &
  8,4 &
  150 &
  0.77271 &
  4,4 &
  150 &
  \textbf{0.7861} &
   \\
Amazon-ratings &
  24492 &
  186100 &
  7.6 &
  0.3757 &
  0.3804 &
  0.1266 &
  -0.0920 &
  8,4 &
  150 &
  0.4776 &
  8,4 &
  147 &
  0.48146 &
  4,4 &
  150 &
  \textbf{0.5130} &
   \\
Minesweeper &
  10000 &
  78804 &
  7.88 &
  0.6829 &
  0.6828 &
  0.0094 &
  0.3915 &
  8,4 &
  74 &
  0.8479 &
  8,4 &
  58 &
  0.8452 &
  4,4 &
  150 &
  \textbf{0.8504} &
   \\
Tolokers &
  11758 &
  1038000 &
  88.28 &
  0.6344 &
  0.5945 &
  0.1801 &
  -0.0803 &
  8,4 &
  37 &
  0.7856 &
  8,4 &
  57 &
  0.78653 &
  4,4 &
  32 &
  \textbf{0.7878} &
   \\
Questions &
  48921 &
  307080 &
  6.28 &
  0.898 &
  0.8396 &
  0.0790 &
  -0.1519 &
  8,4 &
  19 &
  0.9713 &
  8,4 &
  16 &
  0.97145 &
  4,4 &
  17 &
  \textbf{0.9720} &
   \\
Cora &
  2708 &
  10556 &
  3.898 &
  0.8252 &
  0.81 &
  0.7657 &
  -0.0659 &
  8,4 &
  150 &
  0.785 &
  8,4 &
  150 &
  0.75 &
  4,4 &
  150 &
  \textbf{0.7900} &
   \\
CiteSeer &
  3327 &
  9104 &
  2.736 &
  0.7062 &
  0.7355 &
  0.6267 &
  0.0484 &
  8,4 &
  150 &
  0.6670 &
  8,4 &
  150 &
  0.673 &
  4,4 &
  150 &
  \textbf{0.7130} &
   \\
PubMed &
  19717 &
  88648 &
  4.496 &
  0.7924 &
  0.8024 &
  0.6641 &
  -0.0436 &
  8,4 &
  150 &
  0.7610 &
  8,4 &
  150 &
  0.755 &
  4,4 &
  150 &
  \textbf{0.7730} &
   \\
cora &
  19793 &
  126842 &
  6.408 &
  0.5861 &
  0.567 &
  0.4959 &
  -0.045 &
  8,4 &
  150 &
  \textbf{0.7227} &
  8,4 &
  150 &
  0.69942 &
  4,4 &
  150 &
  0.7002 &
   \\
cora\_ml &
  2995 &
  16316 &
  5.448 &
  0.8098 &
  0.7886 &
  0.7401 &
  -0.0721 &
  8,4 &
  150 &
  0.8715 &
  8,4 &
  150 &
  0.86644 &
  4,4 &
  148 &
  \textbf{0.8798} &
   \\
citeseer &
  4230 &
  10674 &
  2.523 &
  0.9577 &
  0.9494 &
  0.9437 &
  -0.0771 &
  8,4 &
  150 &
  \textbf{0.9515} &
  8,4 &
  150 &
  0.94208 &
  4,4 &
  73 &
  \textbf{0.9515} &
   \\
dblp &
  17716 &
  105734 &
  5.968 &
  0.8128 &
  0.8279 &
  0.6522 &
  -0.012 &
  8,4 &
  150 &
  0.8561 &
  8,4 &
  150 &
  0.83973 &
  4,4 &
  66 &
  \textbf{0.8592} &
   \\
pubmed &
  19717 &
  88648 &
  4.496 &
  0.7924 &
  0.8024 &
  0.6641 &
  -0.0436 &
  8,4 &
  150 &
  0.8895 &
  8,4 &
  150 &
  0.88895 &
  4,4 &
  116 &
  \textbf{0.8948} &
   \\
Computers &
  13752 &
  491722 &
  35.76 &
  0.7853 &
  0.7772 &
  0.7002 &
  -0.0565 &
  8,4 &
  150 &
  0.9066 &
  8,4 &
  150 &
  0.90004 &
  4,4 &
  150 &
  \textbf{0.9189} &
   \\
Photo &
  7650 &
  238162 &
  31.13 &
  0.8365 &
  0.8272 &
  0.7722 &
  -0.0449 &
  8,4 &
  150 &
  0.9641 &
  8,4 &
  150 &
  0.95359 &
  4,4 &
  141 &
  \textbf{0.9647} &
   \\
CS &
  18333 &
  163788 &
  8.934 &
  0.832 &
  0.8081 &
  0.7547 &
  0.1126 &
  8,4 &
  47 &
  0.9512 &
  8,4 &
  150 &
  \textbf{0.95882} &
  4,4 &
  46 &
  0.9509 &
   \\
Physics &
  34493 &
  495924 &
  14.38 &
  0.9153 &
  0.9314 &
  0.8474 &
  0.201 &
  8,4 &
  42 &
  0.9677 &
  8,4 &
  150 &
  \textbf{0.96913} &
  4,4 &
  27 &
  0.9680 &
   \\
Flickr &
  89250 &
  899756 &
  10.08 &
  0.3221 &
  0.3195 &
  0.0698 &
  -0.0441 &
  8,4 &
  150 &
  0.4987 &
  8,4 &
  150 &
  0.47847 &
  4,4 &
  125 &
  \textbf{0.5053} &
   \\
Yelp &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  multi-class \\
Reddit &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  large \\
Reddit2 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  large \\
AmazonProducts &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  multi-class
  \\\hline
\end{tabular}
}
\caption{AGS-GNN performance across homophilic and heterophilic graphs}
\label{tab:ags-gsagecheb}
\end{table*}

==> Experiments/GraphSampling.tex <==
%%%%%%%%%%%%%%%%%%
\begin{table*}[!htbp]
\centering
\resizebox{1.0\linewidth}{!}{
\def\arraystretch{1.2}
\begin{tabular}{|l|l|l|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}} &
  \multicolumn{1}{c|}{\textbf{N}} &
  \multicolumn{1}{c|}{\textbf{E}} &
  \textbf{d} &
  \textbf{Whole Graph} &
  \textbf{It.} &
  \textbf{Avg E} &
  \textbf{It} &
  \textbf{Disjoint MST-2} &
  \textbf{Edge reduction} \\ \hline
Cora FULL        & \multicolumn{1}{r|}{19,793} & 126,842 & 6.41  & 0.6598 & 120 & 53171  & 150         & \textbf{0.6608} & 0.58 \\ \hline
Cora             & \multicolumn{1}{r|}{2,708}  & 10,556  & 3.9   & 0.7770 & 59  & 7515   & \textbf{57} & \textbf{0.7868} & 0.29 \\ \hline
citeseer         & 4230                        & 10674   & 2.52  & 0.9492 & 80  & 8802   & 78          & \textbf{0.9530} & 0.18 \\ \hline
CiteSeer         & \multicolumn{1}{r|}{3,327}  & 9,104   & 2.74  & 0.6840 & 62  & 7183   & \textbf{60} & \textbf{0.6896} & 0.21 \\ \hline
Pubmed           & 19717                       & 88648   & 4.5   & 0.7330 & 22  & 48000  & 48          & \textbf{0.7450} & 0.46 \\ \hline
DBLP             & 17716                       & 105734  & 5.97  & 0.8575 & 76  & 46224  & 118         & \textbf{0.8548} & 0.56 \\ \hline
Amazon Computers & 13752                       & 491722  & 35.76 & 0.9200 & 108 & 49942  & 148         & \textbf{0.9213} & 0.90 \\ \hline
Amazon Photos    & 7650                        & 238162  & 31.13 & 0.9647 & 93  & 27825  & 116         & \textbf{0.9643} & 0.88 \\ \hline
Coauthor CS      & 18333                       & 163788  & 8.93  & 0.9534 & 32  & 59110  & 62          & \textbf{0.9540} & 0.64 \\ \hline
Coauthor Physics & 34493                       & 495924  & 14.38 & 0.9685 & 18  & 114951 & 36          & \textbf{0.9688} & 0.77 \\ \hline
\end{tabular}
}
\caption{Disjoint graph Sampling performance on the homophilic graph. The results are average of 5 iterations (for integer data types average values are rounded).}
\label{table:disjointgraph}
\end{table*}
%%%%%%%%%%%%%%%%%%

==> Experiments/NodeSampling.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!htbp]
\centering
\resizebox{0.8\linewidth}{!}{
\def\arraystretch{1.2}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset} &
  \textbf{N} &
  \textbf{E} &
  \textbf{d} &
  \textbf{Rand} &
  \textbf{It.} &
  \textbf{Set.} &
  \textbf{Knn} &
  \textbf{It.} &
  \textbf{Set.} &
  \textbf{Submodular} &
  \textbf{It} \\ \hline
Cora FULL & 19793 & 126842 & 6.41  & 0.6388 & 41  & cos & 0.6461 & \textbf{23} & cos & 0.6128 & 22          \\ \hline
Cora      & 2708  & 10556  & 3.9   & 0.8000 & 33  & cos & 0.7940 & 36          & cos & 0.8100 & \textbf{23} \\ \hline
citeseer  & 4230  & 10674  & 2.52  & 0.9539 & 48  & cos & 0.9444 & \textbf{24} & cos & 0.9433 & 37          \\ \hline
CiteSeer  & 3327  & 9104   & 2.74  & 0.6990 & 150 & cos & 0.6980 & \textbf{27} & cos & 0.7050 & 51          \\ \hline
PubMed    & 19717 & 88648  & 4.5   & 0.7760 & 34  & ecl & 0.7710 & \textbf{22} & ecl & 0.7760 & 25          \\ \hline
dblp      & 17716 & 105734 & 5.97  & 0.8427 & 58  & cos & 0.8496 & 26          & cos & 0.8538 & \textbf{18} \\ \hline
Computers & 13752 & 491722 & 35.76 & 0.8954 & 250 & cos & 0.8742 & 36          & cos & 0.8928 & \textbf{30} \\ \hline
Photo     & 7650  & 238162 & 31.13 & 0.9603 & 204 & cos & 0.9503 & 56          & cos & 0.9614 & \textbf{38} \\ \hline
CS        & 18333 & 163788 & 8.93  & 0.9539 & 18  & cos & 0.9493 & 11          & cos & 0.9534 & \textbf{10} \\ \hline
Physics   & 34493 & 495924 & 14.38 & 0.9664 & 13  & cos & 0.9648 & \textbf{8}  & cos & 0.9656 & \textbf{8}  \\ \hline
\end{tabular}
}
\caption{Performance of Attribute Guided Sampling on homophilic graphs}
\label{tab:homophilic_graph}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Notes.tex <==
\section{Notes}

\subsection{Technical Notes I}
Notes and references for consideration.

\begin{itemize}
    \item $L^+$ as prior-> learnable Sampler -> Sampled graph -> GNN -> prediction
    
    \item shortest path, t-spanner in a subgraph, 
    
    \item Node Sampler, Edge Sampler, Subgraph Sampler, \href{https://cse.msu.edu/~mayao4/dlg_book/chapters/chapter7.pdf}{Sampling methods for GNN}
    
    \item Gumbel-Softmax as a sampler
    
    \item Retain $d^e$ edges for a node of degree d, where $e$ is a parameter that helps control the overall sparsification ratio of the result~\cite{satuluri2011local}. 

    \item Sampling independent edge set such that they do not have any nodes in common~\cite{bravo2019unifying}
    
    \item The the effective resistance based sparsification has the best theoretical properties - favors the retention of edges connecting nodes with few short paths, as such edges have high effective resistance. For clustering application, they often discard such edges, since they distract from the overall cluster structure of the graph~\cite{satuluri2011local}.
    
    
    \item  \cite{batson2013spectral} The effective resistance distance is defined by viewing each edge in a graph as a resistor: an edge of weight w becomes a resistor of resistance 1/w. The entire graph is then viewed as a resistive circuit, and the effective resistance between two vertices is just the electrical resistance in the network between them. It equals the potential difference induced between the vertices when a unit current is injected at one and extracted at the other.\href{https://cacm.acm.org/magazines/2013/8/166320-spectral-sparsification-of-graphs/fulltext}{Reference}
    
    \item It is well-known that $R_e$ is proportional to the commute time between the end-vertices of $e$ and is equal to the probability that e appears in a random spanning tree of G. Spielman and Srivastava~\cite{spielman2011graph} proved that sampling with edge probability pe proportional to $w_eR_e$ is the "right" distribution for creating spectral sparsifiers.
    
    \item Runtime of Lanczos method is $O(dmn)$, $d$ number of non-zero per row, $m$ eigenvalue, eigenvectors, $n$ dimension.[\href{https://en.wikipedia.org/wiki/Lanczos_algorithm#Implementations}{Wiki}]. For graph, $O(\bar{d}k|V|)$, or $O(k|E|)$.
    
    Another, $O(k\times nnz(A)) +O(nk^2)$. Here for graph $nnz(A)==|E|$, thus $O(k|E|)+O(k^2|V|)$. [\href{https://www.chrismusco.com/stableLanczos60.pdf}{MIT review}]
    
    \item Our main idea is to include each edge of G in the sparsifier H with probability proportional to its effective resistance. The effective resistance of an edge is known to be equal to the probability that the edge appears in a random spanning tree of G, and was proven in to be proportional to the commute time between the endpoints of the edge~\cite{spielman2011graph}.
    
    \item Kapralov and Panigrahy showed that one can build a $(1 + \epsilon)$-spectral sparsifier of a graph from the union of spanners of $O(log4 n/\epsilon4)$ random subgraphs of G~\cite{batson2013spectral}.
    
    \item k-neighbors (kN) sparsifier~\cite{sadhanala2016graph} (\href{http://proceedings.mlr.press/v51/sadhanala16.pdf}{Section 3.1})
    
    \item Supervised Graph Sparsifier~\cite{zheng2020robust}
    
    \item Fast graph attention~\cite{srinivasa2020fast}
    
\end{itemize}

\textbf{Research question:} There are many ways to sparsify/condense graph such that the sparsifier preserves certain graph property. For instance, Spectral sparsifiers preserve laplacian eigenvalues, spanners preserve shortest paths, spanning tree preserves connected components. There are many node embedding techniques. Some preserves positional information, others structural information. 
\begin{itemize}
    \item Given a sparsifier $S$ that outputs $G_S$ and embedding technique $B$ that outputs embedding for $B(G(v))$ of vertex $v \in G$, what is the discrepancy between $B(G(v))$ and $B(G_S(v))$? How to quantify it?
    \item How to construct a sparsifier such that given embedding B the discrepancy between $B(G(v))$ and $B(G_S(v))$  is minimised? 
    \item How to construct an embedding $B(G(v))$ such that given a sparsifier $S$ the discrepancy between $B(G(v))$ and $B(G_S(v))$ is minimised? 
    \item How to construct an embedding $B(G(v))$ and a sparsifier $S$ such that the discrepancy between $B(G(v))$ and $B(G_S(v))$ is optimally minimised?
    \item Most sparsifiers are sampling based and are not flexible enough to accomodate a different objective. How to design a flexible sparsifier that can dynamically update its sampling distribution parameter based on the available embedding? 
    \begin{itemize}
        \item See \cite{wickman2021sparrl} for a reinforcement learning based approach. Their objective is to preserve graph topological properties such as PageRank, community structures, and
pairwise shortest path distances. 
    \end{itemize}
    \item Fast Degree preserving sparsification while approximating effective resistance on all edges ($(1 \pm \epsilon)$-approximation): \url{http://ieee-focs.org/FOCS-2018-Papers/pdfs/59f361.pdf}
\end{itemize}

\textcolor{red}{[Naheed:]@Sid, References~\cite{zheng2020robust} and~\cite{wickman2021sparrl} should have plenty of research gaps. Let's read these two papers in details. \\
For instance, the objectives of sparsification are not the same. \textbf{SparRL} sparisifies to preserve various properties. Who said that preserving graph properties is sufficient for a given embedding algorithm to produce a good embedding from the sparse graph?\\
From the point of view of `sparsification objective' \textbf{NeuralSparse} is closer to what we want. Their problem formulation is elegant but their differentiable sampler does not seem to be a good one.
}

\subsection{Technical Notes II}
Some additional notes are...
\begin{itemize}
    \item Cut Approximation
    H approximates G if for every subset $S\in V$ sum of weights of edges leaving S is preserved. 
    
    \item Spectral approximation
    
    \item \href{https://dl.acm.org/doi/pdf/10.1145/3447548.3467361}{Local approximation}
    
    
    
    
\end{itemize}

\subsection{Techinical Notes III}

\begin{itemize}
    \item Compute transition probability of $G,s,k$, compute all pair effective resistance upto $k$ hop from a given $s$. (Computation problems)
    
    \item Exact/approximation effective resistance computation, sublinear time
    
    \item Given $G$ find $H$ that approximates node embedding $f(E(G)-E(H))\le k\epsilon$ (Analysis, novelty) 
    
\end{itemize}

\subsection{Technical Notes III}

\begin{itemize}
    \item Given graph
    \item Find a low-stretch Tree
    \item Decompose the graph into smaller subgraph on the low-stretch tree to increase diameter
    \item random walk of length L
    \item locally approximate the graph
\end{itemize}

\subsection{Technical Notes IV}

\begin{itemize}
    \item drop edges considering node feature
    \item if variance of feature should be increased 
    \item two nodes same feature with high effective resistance low weight even though they have high effective resistance

\end{itemize}


\subsection{Technical Notes V}

\begin{itemize}
    \item Learn kroneckar graph of a graph with feature
    \item Learn the graph structure and feature as well
    
    \item Kroneckar product for graph and as well as features
    
    \item Use those kroneckar product to generate synthetic graphs and train networks
\end{itemize}


\subsection{Technical Notes VI}

\begin{itemize}
    \item spectral sparsification for degree bound constraints
\end{itemize}

\subsection{Technical Notes VII}

\begin{itemize}
    \item spectral sparsification for degree bound constraints
\end{itemize}


\subsection{Links}

\begin{itemize}

    \item \href{https://arxiv.org/pdf/2006.08796.pdf}{Fast GAT}
    
    \item \href{https://arxiv.org/pdf/1902.09702.pdf}{Unify sparsification and coarsening}
    
    \item \href{http://proceedings.mlr.press/v119/zheng20d/zheng20d.pdf}{Supervised Graph Sparsifier}
    
    \item \href{https://scikit-network.readthedocs.io/en/latest/reference/embedding.html}{Scikit Embedding}
    
    \item \href{https://scikit-network.readthedocs.io/en/latest/tutorials/embedding/svd.html}{SVD Scikit}
    
    \item \href{https://docs.scipy.org/doc/scipy/reference/generated/scipy.sparse.linalg.eigsh.html#scipy.sparse.linalg.eigsh}{Scipy Sparse Eigen computation}
    
    \item \href{https://ogb.stanford.edu/docs/leader_linkprop/#ogbl-citation2}{OGB Dataset}
    
    \item \href{https://colab.research.google.com/drive/14OvFnAXggxB8vM4e8vSURUp1TaKnovzX?usp=sharing#scrollTo=pcr9joFQ6Mri}{Colab node classification}
    
    \item \href{https://pytorch-geometric.readthedocs.io/en/latest/modules/datasets.html#torch_geometric.datasets.Planetoid}{Geometric Dataset}
    
    \item \href{https://csustan.csustan.edu/~tom/Clustering/GraphLaplacian-tutorial.pdf}{Graph Laplacian fundamentals}
    
    \item \href{https://appliednetsci.springeropen.com/track/pdf/10.1007/s41109-019-0237-x.pdf}{Learning feature and sturcture via join embedding}
    
    
    \item \href{https://upcommons.upc.edu/bitstream/handle/2117/165548/TFM_GENISFLORIACH.pdf?sequence=1&isAllowed=y}{Low rank approximation for graph based clustering}
    
    \item \href{https://arxiv.org/pdf/1911.04382.pdf}{Graph Spectral sparsification, scalble purtarbation analyis}
    
    \item \href{https://arxiv.org/pdf/0911.4729.pdf}{Hearing the cluster of a graph}
    
    \item \href{https://arxiv.org/pdf/2110.07580.pdf}{Graph condensatation for graph neural network tasks}
    
    \item \href{https://dl.acm.org/doi/pdf/10.1145/1989323.1989399}{Local graph sparsification 2011}
    
    \item \href{https://dl.acm.org/doi/pdf/10.1145/2213556.2213560}{Graph sketches, spanner, subgraph}
    
    \item \href{https://cse.msu.edu/~mayao4/dlg_book/chapters/chapter7.pdf}{Sampling methods GNN}
    
    \item \href{https://www.chrismusco.com/stableLanczos60.pdf}{Lanczos runtime}
    
    \item \href{https://www.cs.cmu.edu/~anupamg/advalgos17/scribes/lec05.pdf}{Distance preserving Tree}
    
    \item \href{https://arxiv.org/pdf/1910.00452.pdf}{Colider Network}
    
    \item \href{https://www.youtube.com/watch?v=qXRs8-LouSQ}{Graph sparsification by effective resistance Youtube}
    
    \item \href{https://dl.acm.org/doi/pdf/10.1145/3447548.3467361}{Local approximation algorithm for Effective resistance}
    
    \item \href{https://arxiv.org/pdf/1805.12051.pdf}{Spectral approximation through Decomposition}
    
    \item \href{https://arxiv.org/pdf/1911.10373.pdf}{GRASPEL: Graph Spectral Learning at Scale}
    
    \item \href{https://arxiv.org/pdf/2006.05929.pdf}{Dataset Condensation with Gradient Matching}
    
    \item \href{https://arxiv.org/pdf/1811.10959.pdf}{Dataset Distillation}

    \item \href{https://csustan.csustan.edu/~tom/Clustering/GraphLaplacian-tutorial.pdf}{Graph Laplacian short tutorial}
    
    \item \href{http://proceedings.mlr.press/v119/zheng20d/zheng20d.pdf}{Neural Sparse}
    
    \item \href{https://arxiv.org/pdf/2106.03476.pdf}{Local algorithm for effective resistance, KDD'21}
    
    \item \href{http://cs-www.cs.yale.edu/homes/spielman/PAPERS/CACMsparse.pdf}{Spectral sprasification theory and application: Spielman}
    
    \item \href{https://arxiv.org/pdf/2112.01565.pdf}{SparRL: Graph sparsification via deep reinforcement learning}
    
    \item \href{http://proceedings.mlr.press/v51/sadhanala16.pdf}{Graph sparsification for laplacian smoothing}
    
    \item \href{https://arxiv.org/pdf/1910.12892.pdf}{Hyperbolic Graph Neural Network}
    
    \item \href{https://arxiv.org/pdf/0803.0929.pdf}{Graph Sparsification by Effective Resistances}
    
    \item \href{https://jmlr.csail.mit.edu/papers/volume13/mahoney12a/mahoney12a.pdf}{A Local Spectral Method for Graphs: With Applications to Improving Graph Partitions and Exploring Data Graphs Locally}
    
    \item \href{https://arxiv.org/pdf/1805.12051.pdf}{Graph Sparsification, Spectral Sketches, and Faster Resistance Computation, via Short Cycle Decompositions}
    
    \item \href{https://arxiv.org/pdf/1206.5180.pdf}{INVERTIBILITY OF RANDOM MATRICES: UNITARY AND
ORTHOGONAL PERTURBATIONS}
    
    \item \href{https://arxiv.org/pdf/0808.0163.pdf}{Twice Ramanujon sparsifier}
    
    \item  \href{https://www.cs.princeton.edu/~chazelle/pubs/DeterminRandomSampling.pdf}{Deterministic RandomSampling}
    
    \item \href{https://link.springer.com/content/pdf/10.1007/s41060-016-0020-3.pdf}{A greedy algorithm to construct sparse graph by using ranked dictionary}
    
    \item \href{https://en.wikipedia.org/wiki/Monte_Carlo_tree_search}{Monte Carlo tree search tree}
    
    \item \href{https://aclanthology.org/W11-0318.pdf}{Mututal K-nn for graph construction}
    
    \item \href{https://arxiv.org/pdf/2110.07580.pdf#cite.wang2018dataset}{Graph Condensation for Graph Neural Network}
    
    \item \href{https://arxiv.org/pdf/1612.04883.pdf}{Graph Summarization Methods and Applications: A Survey}
    
    \item \href{http://proceedings.mlr.press/v80/norouzi-fard18a/norouzi-fard18a.pdf}{beyond 1/2-Approximation for Submodular Maximization}
\end{itemize}


==> key-result-saved.tex <==

In this subsection, we provide our key results by means of performance profiles that compare the \ags{} algorithm against the best-performing algorithms for both homophilic and heterophilic classes of graphs. 
%In this section, we summarize key results using 
In a performance profile, algorithms are compared on how they perform on a collection of problems, and the profile summarizes an algorithm's performance on the collection. 
The Y-axis shows the fraction of problems solved by an algorithm when the $F_1$-score (in percentage) can deviate by a certain factor relative to the best-performing algorithm for those problems. 
The X-axis represents the deviation in $F_1$-score relative to the best-performing algorithm.%by which a given algorithm  fares relative to the best performing algorithm  for that particular input, and the Y-axis represents the fraction of problems solved using . 
The closer a curve (algorithm) is to the Y-axis, and the earlier it reaches $100\%$, the better is its performance w.r.t. other algorithms across all the problems considered.
For example, Fig.~\ref{fig:smallhetero} summarizes results from five algorithms across 17 test problems for small heterophilic graphs. The X-axis represents the deviation in $F_1$-score relative to the best-performing algorithm, and the Y-axis represents the fraction of 17 problems solved using that value of the $F_1$ score.  we observe that \ags{} performs the best or close-to-best for about $50\%$ of the problems, and has up to $10\%$ lower $F_1$ scores compared to the best algorithm for about $50\% $ of the problems. In contrast, LINKX has about $35\% $ lower $F_1$-scores for about $20\% $ of the problems, but has small deviation for about $80\% $ of the problems. \looseness=-1
%Thus, for most small heterophilic graphs, ACM-GCN, \agsns{}, and LINKX are the best algorithms with slight edges to \agsns{} and ACM-GCN. GSAGE and GSAINT perform similarly.
%
%Figure~\ref{fig:perfplot} shows performance plots comparing \ags{} with other methods, while detailed results with numerical values are provided in Appendix (Tables~\ref{tab:smallhetero}, \ref{tab:smallhomophilic}).


%The performance plot, in Fig.~\ref{fig:perfplot}, compares algorithms across various test problems, where the $x$-axis represents the deviation in $F_1$-score relative to the best-performing algorithm and the $y$-axis indicates the percentage of problems each algorithm excels on. Each algorithm is plotted based on its deviation in $F_1$-score and the corresponding percentage of problems on which it performs best. The ranking is determined by identifying the algorithm with the highest percentage of problems solved, showcasing consistency across diverse scenarios. 
%For example, in Fig.~\ref{fig:smallhetero} of small heterophilic graphs, we can see ACM-GCN, \agsns{}, and LINKX are the top three performing algorithms for $80\%$ of the problems where \agsns{} is leading up to $90\%$. In some problems (e.g., \texttt{squirrel}), LINKX performed poorly (about $35\%$ deviation in $F_1$ measure from the best performer AGM-GCN) relative to others and pushed it to the end when all problems ($100\%$) are considered. 
%\smf{In \cref{fig:perfplot}, is the x-axis is also a percentage of deviation? y-axis title: fraction->percentage. One alternative is to instead of showing percentage of problems solved in y-axis, show actual number of problems solved.  }

%\Sid{Yes. updated}


%The performance plot, in Fig.~\ref{fig:perfplot}, compares five algorithms across various test problems, where the $x$-axis represents the deviation in $F_1$-score relative to the best-performing algorithm and the $y$-axis indicates the percentage of problems each algorithm solves within this deviation in accuracy. In other words, given a bound on quality, we ask how many problems are being solved by the competing methods. For a particular algorithm, as we relax the bound, the more problems are solved. 
%It is apparent that the algorithms that completes all the problems ($100\%$ in the $y$-axis) within small deviation of accuracy (in $x$-axis) are better than those who requires large deviation. For small heterophilic graphs (Fig.~\ref{fig:smallhetero}), we see ACM-GCN, \agsns{}, and LINKX are the top three performing algorithms for $80\%$ of the problems whereas \agsns{} is leading up to $90\%$. 
%In a few problems (e.g., \texttt{squirrel}), LINKX performed significantly worse (about $35\%$ deviation in $F_1$ measure from the best performer AGM-GCN) than the others, and that made LINKX complete last, despite solving most of the instances ($80\%$) within small deviation ($\leq 5$). %pushed it to the end when all problems ($100\%$) are considered  

For large heterophilic graphs (Fig.~\ref{fig:largehetero}),  performance improvements for \agsns{} is considerably better than all algorithms. LINKX$+$ performs second-best for $75\%$ of the problems.
In small homophilic graphs (Fig.~\ref{fig:smallhomo}), \agsns{} and GSAGE are the top two performers for most of the problems, followed by GSAINT, ACM-GCN, and LINKX. This is expected since ACM-GCN and LINKX are tailored for heterophilic graphs. In large homophilic graphs (Fig.~\ref{fig:largehomo}), \agsns{} is the best-performing algorithm in terms of accuracy, followed by GSAGE. We also observe from this figure that for homophilic graphs, LINKX$+$ is not competitive.
In Table.~\ref{tab:smallothergnns} (Appendix~\ref{subsec:othermethods}) we present  performance of \agsns{} compared to $18$ recent competing algorithms on small heterophilic graphs. We observe that ACM-GCN, \agsns{}, and LINKX remain the best-performing, with \agsns{} as the leading method for these inputs.


The full set of results with numerical values are provided in Appendix (Tables~\ref{tab:smallhetero},~\ref{tab:smallhomophilic},~\ref{tab:large_heterophilic_graphs},~\ref{tab:large_homophilic_graphs},~\ref{tab:smallothergnns}). 
These tables present the mean ($\mu$) and standard deviation ($\sigma$) of the runs. We use a one-tailed statistical hypothesis $t$-test to verify whether one set of values is better than the other. The better-performing results are highlighted in boldface.


==> preamble.tex <==
\usepackage{geometry}
% \geometry{letterpaper,textwidth=350pt,textheight=680pt,tmargin=60pt,
%             left=72pt,footskip=24pt,headsep=18pt,headheight=14pt}
\RequirePackage{amsmath}
\usepackage{amssymb}
\usepackage{textcase}
\usepackage{soul}
\usepackage{indentfirst}
\crefname{section}{\S}{\S\S}
\crefname{subsection}{\S}{\S\S}
\newtheorem{theorem}{Theorem}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
    pdftitle={Overleaf Example},
    pdfpagemode=FullScreen,
    }

\urlstyle{same}

\usepackage{enumitem,kantlipsum}

\newcommand{\eps}{\varepsilon}
\newcommand{\kron}{\otimes}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\tvec}{vec}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\tspan}{span}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator{\subjectto}{subject\ to}

\newcommand{\mat}[1]{\boldsymbol{#1}}
\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\vecalt}[1]{\boldsymbol{#1}}

\newcommand{\conj}[1]{\overline{#1}}

\newcommand{\normof}[1]{\|#1\|}
\newcommand{\onormof}[2]{\|#1\|_{#2}}

\newcommand{\MIN}[2]{\begin{array}{ll} \displaystyle \minimize_{#1} & {#2} \end{array}}
\newcommand{\MINone}[3]{\begin{array}{ll} \displaystyle \minimize_{#1} & {#2} \\ \subjectto & {#3} \end{array}}
\newcommand{\OPTone}{\MINone}
\newcommand{\MINthree}[5]{\begin{array}{ll} \displaystyle \minimize_{#1} & {#2} \\ \subjectto & {#3} \\ & {#4} \\ & {#5} \end{array}}

\newcommand{\MAX}[2]{\begin{array}{ll} \displaystyle \maximize_{#1} & {#2} \end{array}}
\newcommand{\MAXone}[3]{\begin{array}{ll} \displaystyle \maximize_{#1} & {#2} \\ \subjectto & {#3} \end{array}}


\newcommand{\itr}[2]{#1^{(#2)}}
\newcommand{\itn}[1]{^{(#1)}}

\newcommand{\prob}{\mathbb{P}}
\newcommand{\probof}[1]{\prob\left\{ #1 \right\}}

\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\spmat}[1]{\left(\begin{smallmatrix} #1 \end{smallmatrix}\right)}
\newcommand{\sbmat}[1]{\left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}

\providecommand{\eye}{\mat{I}}
\providecommand{\mA}{\ensuremath{\mat{A}}}
\providecommand{\mB}{\ensuremath{\mat{B}}}
\providecommand{\mC}{\ensuremath{\mat{C}}}
\providecommand{\mD}{\ensuremath{\mat{D}}}
\providecommand{\mE}{\ensuremath{\mat{E}}}
\providecommand{\mF}{\ensuremath{\mat{F}}}
\providecommand{\mG}{\ensuremath{\mat{G}}}
\providecommand{\mH}{\ensuremath{\mat{H}}}
\providecommand{\mI}{\ensuremath{\mat{I}}}
\providecommand{\mJ}{\ensuremath{\mat{J}}}
\providecommand{\mK}{\ensuremath{\mat{K}}}
\providecommand{\mL}{\ensuremath{\mat{L}}}
\providecommand{\mM}{\ensuremath{\mat{M}}}
\providecommand{\mN}{\ensuremath{\mat{N}}}
\providecommand{\mO}{\ensuremath{\mat{O}}}
\providecommand{\mP}{\ensuremath{\mat{P}}}
\providecommand{\mQ}{\ensuremath{\mat{Q}}}
\providecommand{\mR}{\ensuremath{\mat{R}}}
\providecommand{\mS}{\ensuremath{\mat{S}}}
\providecommand{\mT}{\ensuremath{\mat{T}}}
\providecommand{\mU}{\ensuremath{\mat{U}}}
\providecommand{\mV}{\ensuremath{\mat{V}}}
\providecommand{\mW}{\ensuremath{\mat{W}}}
\providecommand{\mX}{\ensuremath{\mat{X}}}
\providecommand{\mY}{\ensuremath{\mat{Y}}}
\providecommand{\mZ}{\ensuremath{\mat{Z}}}
\providecommand{\mLambda}{\ensuremath{\mat{\Lambda}}}
\providecommand{\mSigma}{\ensuremath{\mat{\Sigma}}}
\providecommand{\mPbar}{\bar{\mP}}

\providecommand{\ones}{\vec{e}}
\providecommand{\va}{\ensuremath{\vec{a}}}
\providecommand{\vb}{\ensuremath{\vec{b}}}
\providecommand{\vc}{\ensuremath{\vec{c}}}
\providecommand{\vd}{\ensuremath{\vec{d}}}
\providecommand{\ve}{\ensuremath{\vec{e}}}
\providecommand{\vf}{\ensuremath{\vec{f}}}
\providecommand{\vg}{\ensuremath{\vec{g}}}
\providecommand{\vh}{\ensuremath{\vec{h}}}
\providecommand{\vi}{\ensuremath{\vec{i}}}
\providecommand{\vj}{\ensuremath{\vec{j}}}
\providecommand{\vk}{\ensuremath{\vec{k}}}
\providecommand{\vl}{\ensuremath{\vec{l}}}
\providecommand{\vm}{\ensuremath{\vec{l}}}
\providecommand{\vn}{\ensuremath{\vec{n}}}
\providecommand{\vo}{\ensuremath{\vec{o}}}
\providecommand{\vp}{\ensuremath{\vec{p}}}
\providecommand{\vq}{\ensuremath{\vec{q}}}
\providecommand{\vr}{\ensuremath{\vec{r}}}
\providecommand{\vs}{\ensuremath{\vec{s}}}
\providecommand{\vt}{\ensuremath{\vec{t}}}
\providecommand{\vu}{\ensuremath{\vec{u}}}
\providecommand{\vv}{\ensuremath{\vec{v}}}
\providecommand{\vw}{\ensuremath{\vec{w}}}
\providecommand{\vx}{\ensuremath{\vec{x}}}
\providecommand{\vy}{\ensuremath{\vec{y}}}
\providecommand{\vz}{\ensuremath{\vec{z}}}
\providecommand{\vpi}{\ensuremath{\vecalt{\pi}}}

\providecommand{\vlambda}{\ensuremath{\vecalt{\lambda}}}


% \sodef\allcapsspacing{\upshape}{0.15em}{0.65em}{0.6em}%
% NAHEED macro
\newcommand{\naheed}[1]{\textcolor{blue}{[NAHEED: #1]}}


%--Annotation----
\newcommand{\SMF}[2][inline]{\todo[color=cyan!50,#1]{\sf \textbf{Ferdous:} #2}\xspace}
\newcommandx{\smf}[2][1=]{\todo[color=cyan!50,#1]{\sf \textbf{smf:} #2}\xspace}


==> working-comments-smf.tex <==
1. We may define high and low pass filters upfront in the paper since it is used heavily.

